Angular Luminance for Material Segmentation

Moving cameras provide multiple intensity measurements per pixel, yet often semantic segmentation, material recognition, and object recognition do not utilize this information. With basic alignment over several frames of a moving camera sequence, a distribution of intensities over multiple angles is obtained. It is well known from prior work that luminance histograms and the statistics of natural images provide a strong material recognition cue. We utilize per-pixel {\it angular luminance distributions} as a key feature in discriminating the material of the surface. The angle-space sampling in a multiview satellite image sequence is an unstructured sampling of the underlying reflectance function of the material. For real-world materials there is significant intra-class variation that can be managed by building a angular luminance network (AngLNet). This network combines angular reflectance cues from multiple images with spatial cues as input to fully convolutional networks for material segmentation. We demonstrate the increased performance of AngLNet over prior state-of-the-art in material segmentation from satellite imagery.

==> related_work.tex <==



%semantic segmentation for hyperspectral images
Models based on Fully Convolutional Neural Networks (FCN) \cite{long2015fully} have demonstrated superior performance on several segmentation benchmarks \cite{zhou2017scene, everingham2010pascal, cordts2016cityscapes}. When adapting the CNNs \cite{he2016deep, krizhevsky2012imagenet, simonyan2014very} deployed for the task of image classification into segmentation,   a coarse-to-fine deconvolution network is learned for upsampling \cite{noh2015learning, badrinarayanan2015segnet, chen2018encoder, chen2017rethinking}. For example, DeepLabv3+ \cite{chen2018encoder} extends DeepLabv3 \cite{chen2017rethinking} by adding a decoder module to recover the object boundaries.
To enforce prediction consistency during the coarse-to-fine deconvolution, a hierarchical supervision is introduced to help optimize the learning process \cite{fu2017stacked, zhao2017icnet}. Inspired by this work, we use a similar hierarchical supervision module that combines angular histograms with image features at different upsampling scales during the coarse-to-fine deconvolution. 
Recently, PSPNet \cite{zhao2017pyramid} and EncNet \cite{zhang2018context} leverage global context information and boost segmentation performance dramatically. However, for material segmentation,  the global context information  often provides limited help in cases where the same semantic object can be composed of different materials. 
Indeed, our comparison results in Section~\ref{sec:experiments} indicate that the context information of PSPNet and EncNet do not boost performance over FCN for the task of material segmentation. 
%In cases where many materials map to the same object, global context information is not helpful to distinguish material classes from the same semantic objects. We prove our assumption in the experiment section.

For multiview segmentation, Ma \etal enforce the prediction consistency by warping CNN feature maps from multiple views into a common reference \cite{ma2017multi}. For this work, the segmentation is constrained to be consistent over all views. Our approach has an important distinction in its use of multiview images. Instead of consistency, we consider the per-pixel vector of intensities as a sampling of the underlying BRDF from unknown viewing and illumination angles. This unstructured sampling of reflectance information is a physically meaningful cue for material id. 
%Qi \etal use 3D renderings of the multiview objects for 3D segmentation \cite{qi2017pointnet}. However, the image 3D rendering is a time and memory consuming process. 
%In this paper, we experiment with a different approach that building the angular histogram to characterize material appearance difference for multiview material segmentation.

\iffalse
\begin{figure}[t]
\centering
\includegraphics[width= \linewidth]{figure/data_pixel.png}
\caption{Number of annotated pixels (y-aixs) per class and their associated categories (x-aixs) for the labeled satellite material segmentation dataset.}
\label{fig:data_pixel}
%\vspace{-0.1in}
\end{figure}
\fi

%BRDF and Representing data with histogram dstribution
Material radiometric properties are captured by the bidirectional reflectance distribution function (BRDF) \cite{NicoBRDF} and the many variants including the bidirectional texture function (BTF) \cite{dana1999reflectance}, svBRDF\cite{lensch2001image}, BSSRDF\cite{jensen2001practical}. Using intensity  distributions or {\it luminance histograms} to represent reflectance variations has been explored in several previous works \cite{dror2001estimating, Adelson01, shell2004novel,simoncelli2001natural, motoyoshi2007image}. Motoyoshi \etal showed that the skewness of the luminance histogram and the skewness of sub-band filter outputs are correlated with surface gloss and inversely correlated with surface albedo (diffuse reflectance) \cite{motoyoshi2007image}. Dror \etal  employs histogram statistics to estimate surface reflectance from a single image \cite{dror2001estimating}. Recently, Wang \etal propose a learnable histogram layer and learn histogram features within deep neural networks in end-to-end training \cite{wang2016learnable}. Inspired by both classic and recent work, we employ the  angular histogram  to represent  material reflectance in material segmentation networks. While prior work computes image statistics over a fixed spatial region, our approach computes statistics over multiple viewing angles for each pixel (or for each superpixel region).  

%For example, the classic luminance histogram is computed over the entire image or over a fixed size patch. Our  angular histogram is computed over multiple views  that was assumed to be the same material, our approach uses per-pixel (or per superpixel) statistics requiring no assumption of a  spatially uniform material within a large fixed region. composition and no apriori material segmentation.  


\iffalse
\begin{figure}[t]
\centering
\includegraphics[width= \linewidth]{figure/superpixel_acc.png}
\caption{Oracle superpixel quantization performance for the test regions (Jacksonville and Omaha). The average achievable segmentation pixel accuracy (pixelAcc, Left) and mean Intersection of Union (mIoU, Right) with the varying number of superpixels for the satellite dataset.}
\label{fig:superpixel_acc}
%\vspace{-0.1in}
\end{figure}
\fi
